Speech Representation Analysis based on Inter- and Intra-Model Similarities

Self-supervised models have revolutionized speech processing, achieving new levels of performance in a wide variety of tasks with limited resources. However, the inner workings of these models are still opaque. In this paper, we aim to analyze the encoded contextual representation of these foundation models based on their inter- and intra-model similarity, independent of any external annotation and task-specific constraint. We examine different SSL models varying their training paradigm -- Contrastive (Wav2Vec2.0) and Predictive models (HuBERT); and model sizes (base and large). We explore these models on different levels of localization/distributivity of information including (i) individual neurons; (ii) layer representation; (iii) attention weights and (iv) compare the representations with their finetuned counterparts.Our results highlight that these models converge to similar representation subspaces but not to similar neuron-localized concepts\footnote{A concept represents a coherent fragment of knowledge, such as ``a class containing certain objects as elements, where the objects have certain properties. We made the code publicly available for facilitating further research, we publicly released our code.

==> table.tex <==
\begin{table}[]
\centering
% \renewcommand{\arraystretch}{0.8}
% \vspace{-1.6cm}
\scalebox{1.}{
\begin{tabular}{lccc}
\toprule
Dataset & F1 $\uparrow$ & FRR $\downarrow$ & PER $\downarrow$\\ \toprule
\midrule
\rowcolor{blue!10}
\multicolumn{4}{c}{Monolingual {\em vs} Multilingual} \\\midrule
\midrule
\multicolumn{4}{c}{Mono} \\
\midrule

L2-Artic & 56.42\% & 6.30\% & 14.13 \\
LATIC & 56.13\% & 7.25\% & 9.27 \\
AraVoiceL2 v2 & 76.91\% & 3.95\% & 7.39 \\
\midrule

\multicolumn{4}{c}{Mono:$<\mathfrak{p}>$} \\ \midrule
L2-Artic & \underline{57.37}\% & 5.61\% & 13.46 \\
LATIC & 73.91\% & 3.11\% & 4.61 \\
AraVoiceL2v2 & \underline{77.73}\% & 2.93\% & 7.03 \\

\midrule
\multicolumn{4}{c}{Multi} \\
\midrule

L2-Artic & 54.40\% & 5.76\% & 13.99 \\
LATIC & 54.40\% & 7.82\% & 10.16 \\
AraVoiceL2v2 & 75.86\% & 3.74\% & 7.42 \\
\midrule
\multicolumn{4}{c}{Multi:$<\mathfrak{p}>$} \\ \midrule
L2-Artic & 55.81\% & 5.46\% & 13.70 \\
LATIC & 66.84\% & 4.25\% & 6.36 \\
AraVoiceL2v2 & 71.76\% & 4.62\% & 10.96 \\ \midrule
% \midrule
\multicolumn{4}{c}{Multi:$<\mathfrak{p}, \mathbb{O}(L2)>$} \\ \midrule
L2-Artic & 55.98\% & \underline{5.10}\% & \underline{13.29} \\
LATIC & \underline{75.65}\% & \underline{2.54}\% & \underline{4.11} \\
AraVoiceL2v2 & 76.88\% & \underline{2.46}\% & \underline{6.86} \\
\midrule\midrule
\rowcolor{green!10}
\multicolumn{4}{c}{Proposed L1-aware Multi:One-hot Embed. (topline)} \\
\midrule
% \midrule
% \multicolumn{4}{c}{Multi:$<\mathfrak{p}, \mathbb{O}(L1)>$} \\ \midrule
% \multicolumn{4}{c}{Multilingual:$<\mathfrak{p}>$} \\ \midrule
% L2-Artic & 55.81\% & 5.46\% & 13.70 \\
% LATIC & 66.84\% & 4.25\% & 6.36 \\
% AraVoiceL2 v2 & 71.76\% & 4.62\% & 10.96 \\ \midrule
% \multicolumn{4}{c}{Multilingual:$<\mathfrak{p}, \mathbb{O}(L1)>$} \\ \midrule
% L2-Artic & 55.98\% & 5.10\% & 13.29 \\
% LATIC & 75.65\% & 2.54\% & 4.11 \\
% AraVoiceL2 v2 & 76.88\% & 2.46\% & 6.86 \\
\midrule
\multicolumn{4}{c}{L1-Multi:$<\mathfrak{p},\mathbb{O}(L1)>$} \\\midrule
L2-Artic & \textit{57.14}\% & 4.56\% & 12.66 \\
LATIC & \textbf{75.96}\% & 2.32\% & \textbf{3.92} \\
AraVoiceL2v2 & 76.28\% & 2.31\% & 6.80 \\\midrule
\multicolumn{4}{c}{L1-Multi:$<\mathfrak{p},\mathbb{O}(L1,L2)>$} \\\midrule
L2-Artic & 57.12\% & \textbf{4.26}\% & \textbf{12.52} \\
LATIC & 75.77\% & \textit{2.27}\% & 3.93 \\
AraVoiceL2v2 & \textit{78.00}\% & \textbf{2.03}\% & \textit{6.42} \\\midrule
\midrule
\rowcolor{green!10}
\multicolumn{4}{c}{Proposed L1-aware Multi:Aux Embed.} \\\midrule
\midrule
\multicolumn{4}{c}{L1-Multi:$<\mathfrak{p},\varepsilon>$ (Sequential)} \\\midrule
\rowcolor{yellow!20}
L2-Artic & \textbf{57.40}\% & 4.60\% & 12.55 \\
\rowcolor{yellow!20}
LATIC & 74.82\% & 2.45\% & 4.19 \\
\rowcolor{yellow!20}
AraVoiceL2v2 & \textbf{78.42}\% & 2.25\% & \textbf{6.13 }\\\midrule
\multicolumn{4}{c}{L1-Multi:$<\mathfrak{p},\varepsilon^*>$ (Joint)} \\\midrule
L2-Artic & 56.87\% & 4.87\% & 12.92 \\
LATIC & \textit{75.34}\% & \textbf{2.23}\% & 4.38 \\
AraVoiceL2v2 & 76.44\% & 2.27\% & 6.35 \\
\bottomrule
\end{tabular}}
\vspace{-0.2cm}
\caption{\small{Results for different experimental settings. $<\mathfrak{p}>$ represent phoneme embedding, $<\mathbb{O}(L_*)>$: indicate one-hot $L_*$. Auxiliary (Aux.) network training sequentially ($<\varepsilon>$) or jointly ($<\varepsilon^*>$). topline: best-case scenario knowing all possible L1s. Green rows highlight our proposed frameworks; bold values are best for each dataset/metric.
}}
\vspace{-1.6cm}
\label{tab:seen_rslt}
\end{table}


==> tmp.tex <==
The phonological discrepancies between a speaker's native language (L1) and the target language (L2) serves as a major factor for mispronunciation. Traditionally designing mispronunciation detecting and diagnosis (MDD) often focus solely on L2-data for a single target language, hence neglecting the valuable insights that could be captured from multilingual target language modeling and L1-aware features. 

Therefore, this paper introduces a novel multilingual MDD (multi-MMD) architecture enriched with L1-aware speech representation. 
Using the L1-dependent multilingual latent space, the model learns to capture the nuanced influences of the speaker's phonological background while being sensitive to the idiosyncrasies of each target language.
The multi-MMD model trained 



Utilizing an end-to-end transformer-based speech encoder architecture, the model is optimized in an end-to-end manner utilizing 
a unified multilingual phoneme output space. This is further augmented by embedding both L1 and L2 speech characteristics, which are solely extracted from the raw input speech, thereby offering a holistic approach to pronunciation assessment.

% become more sensitive to the idiosyncrasies of each language.
% capturing the nuanced influences of the speaker's linguistic background, thereby offering a more robust and comprehensive approach to pronunciation error detection in low-resource setting.

% that primarily supports English, Arabic, and Mandarin as target languages. This framework is enriched with L1-aware speech representation, capturing the nuanced influences of the speaker's linguistic background, thereby offering a more robust and comprehensive approach to pronunciation error detection in low-resource setting.


We demonstrates the generalizability using unseen datasets EpaDB, Speechocean762.


Our experiments shows that L1-dependent multilingual latent space able to capture 


the nuanced influences of the speaker's phonological background while being sensitive to the idiosyncrasies of each target language.


The multi-MDD is then optimized jointly for a unified phoneme output space for the following target languages --  English, Arabic, and Mandarin.

These results in a L1-dependent multilingual latent space and the model learns to capture the nuanced influences of the speaker's phonological background while being sensitive to the idiosyncrasies of each target language.


% We trained an end-to-end transformer-based speech encoder with an unified multilingual phoneme output space. further enriched with L1- and L2-speech embedding extracted from the raw input speech only. 


% his is further augmented by embedding both L1 and L2 speech characteristics, which are solely extracted from the raw input speech, thereby offering a holistic approach to pronunciation assessment.




An unified phoneme set is designed to train a transformer-based speech encoder that is further enriched with L1- and L2-speech embedding trained in an end-to-end manner. 


The framework is optimised 

phonetic representation is designed to train The multi-MMD model trained 



% Mispronunciation often result from contrasting phonological patterns between a speaker's native language (L1) and the target language (L2). 
The phonological discrepancies between the speaker's native language (L1) and the target language (L2) is one of the primary factors in mispronunciation. These contrasting patterns are often missing when modeling mispronunciation detection model using the available L2-data for a single target language overlooking the potential in multilingual target language modeling and L1-aware representations. This paper proposes a novel multilingual MDD architecture -- supporting mainly English, Arabic, and Mandarin, as target language.
% enhanced with L1-aware speech representation to characterize the intricacies of each target language phonology influenced by speakers' own nativity. 
% Our method enriches this paradigm by 
The proposed multilingual framework is enhanced with L1-aware speech representation, encapsulating the influence of speaker's own nativity.  

phonological patterns to enhance the robustness and accuracy of mispronunciation detection in multiple languages.
% along with lack of L2-data for the target language.
The paper proposes a novel multilingual MDD architecture that







% .  We demonstrates the generalizability using unseen datasets EpaDB, Speechocean762.


% Our experiments shows that L1-dependent multilingual latent space able to capture 


% the nuanced influences of the speaker's phonological background while being sensitive to the idiosyncrasies of each target language.


% The multi-MDD is then optimized jointly for a unified phoneme output space for the following target languages --  English, Arabic, and Mandarin.

% These results in a L1-dependent multilingual latent space and the model learns to capture the nuanced influences of the speaker's phonological background while being sensitive to the idiosyncrasies of each target language.


% % We trained an end-to-end transformer-based speech encoder with an unified multilingual phoneme output space. further enriched with L1- and L2-speech embedding extracted from the raw input speech only. 


% % his is further augmented by embedding both L1 and L2 speech characteristics, which are solely extracted from the raw input speech, thereby offering a holistic approach to pronunciation assessment.




% An unified phoneme set is designed to train a transformer-based speech encoder that is further enriched with L1- and L2-speech embedding trained in an end-to-end manner. 


% The framework is optimised 

% phonetic representation is designed to train The multi-MMD model trained 



% % Mispronunciation often result from contrasting phonological patterns between a speaker's native language (L1) and the target language (L2). 
% The phonological discrepancies between the speaker's native language (L1) and the target language (L2) is one of the primary factors in mispronunciation. These contrasting patterns are often missing when modeling mispronunciation detection model using the available L2-data for a single target language overlooking the potential in multilingual target language modeling and L1-aware representations. This paper proposes a novel multilingual MDD architecture -- supporting mainly English, Arabic, and Mandarin, as target language.
% % enhanced with L1-aware speech representation to characterize the intricacies of each target language phonology influenced by speakers' own nativity. 
% % Our method enriches this paradigm by 
% The proposed multilingual framework is enhanced with L1-aware speech representation, encapsulating the influence of speaker's own nativity.  

% phonological patterns to enhance the robustness and accuracy of mispronunciation detection in multiple languages.
% % along with lack of L2-data for the target language.
% The paper proposes a novel multilingual MDD architecture that 
